CPU and GPU Accelerated Fully Homomorphic Encryption

Fully Homomorphic Encryption (FHE) is one of the most promising technologies for privacy protection as it allows an arbitrary number of function computations over encrypted data. However, the computational cost of these FHE systems limits their widespread applications. In this paper, our objective is to improve the performance of FHE schemes by designing efficient parallel frameworks. In particular, we choose Torus Fully Homomorphic Encryption (TFHE) as it offers exact results for an infinite number of boolean gate (e.g., AND, XOR) evaluations. We first extend the gate operations to algebraic circuits such as addition, multiplication, and their vector and matrix equivalents. Secondly, we consider the multi-core CPUs to improve the efficiency of both the gate and the arithmetic operations. Finally, we port the TFHE to the Graphics Processing Units (GPU) and device novel optimizations for boolean and arithmetic circuits employing the multitude of cores. We also experimentally analyze both the CPU and GPU parallel frameworks for different numeric representations (16 to 32-bit). Our GPU implementation outperforms the existing technique, and it achieves a speedup of 20x for any 32-bit boolean operation and 14.5x for multiplications.

==> Tables/FHEcomparativeAnalysis.tex <==
% \begin{table*}[]
% \centering
% \caption{A comparative analysis of existing FHE schemes}
% \label{tbl:comparativeAna}
% \begin{tabular}{l|l|l|l|l|l}
% \hline
%                     & FV   & TFHE      & HEEAN        & SEAL & TFHE(GPU) \\ \hline
% Year                & 2012 & 2016      & 2018         & 2019 &     \\ \hline
% Cryptosystem        &      & GSW       &              &      &           \\ \hline
% Bit Security        &      & 110 & 110    &      & 110 \\ \hline
% Size (KB)           &      & 31.5      & 16896.02     &      & 31.5      \\ \hline
% Addition (ms)       &      & 2631.08   & 16.06        &      & 1487.02   \\ \hline
% Multiplication (ms) &      & 49853.98  & 1076.53      &      & 10218.28  \\ \hline
% Parallelism         & No   & No        & CPU level &      & GPU       \\ \hline
% Bootstrapping       & No   & Exact     & Approx.  &      & Exact     \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \caption{A comparative analysis of existing FHE schemes for different parameters on 32-bit number.}
% \label{tbl:comparativeAna}
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
% \hline
%           & Year   & Cryptosystem & Bit security & Size (kb) & Addition (ms) & Multiplication (ms) & Parallelism & Bootstrapping \\ \hline
% FV-NFLlib~\cite{fan2012somewhat} & 2012   & FV           & 127    & 512       & 0.065         & 41                  & No          & No            \\ \hline
% TFHE~\cite{chillotti2016faster}      & 2016   & GSW          & 110    & 31.5      & 2,631.08       & 49,853.98            & AVX~\cite{lomont2011introduction}         & Exact         \\ \hline
% HEEAN~\cite{cheon2018bootstrapping}     & 2018   & CKKS         & 157    & 7,168      & 5.096         & 1,214.86             & CPU        & Approximate   \\ \hline
% SEAL~\cite{sealcrypto}      & 2019   & BFV          & 157    & 8,806.4    & 4,237          & 23,954               & No          & No            \\ \hline
% TFHE (GPU) &  & GSW          & 110    & 31.5      & 1,487.02       & 10,218.28            & GPU         & Exact         \\ \hline
% \end{tabular}
% \end{table*}

\begin{table*}[t]

\centering
% \color{blue}
\caption{A comparative analysis of existing Homomorphic Encryption schemes for different parameters on 32-bit number.}
% \renewcommand{\arraystretch}{1.1}
\label{tbl:comparativeAna}
% \begin{adjustbox}{max width=\linewidth}
\resizebox{\linewidth}{!}{
\begingroup
% \renewcommand*{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
                                                          & \textbf{Year}   & \textbf{Homomorphism}   & \textbf{Bootstrapping}         & \textbf{Parallelism}                                             & \textbf{Bit security} & \textbf{Size (kb)} & \textbf{Add. (ms)}         & \textbf{Mult. (ms)}  \\ \hline 
RSA~\cite{rivest1978method}         & 1978   & Partial & $\times$ & $\times$                                   &    128          &      0.9    & $\times$ &          5            \\ \hline
Paillier~\cite{paillier1999public}  & 1999   & Partial       & $\times$ & $\times$                                   &  128            &  0.3 &   4 & $\times$ \\ \hline
% FV-NFLlib~\cite{fan2012somewhat}    & 2012   & Somewhat       & $\times$ & $\times$                                   & 127    & 512       & 0.065                 & 41                   \\ \hline
TFHE~\cite{chillotti2016faster}     & 2016   & Fully          & Exact                 & AVX~\cite{lomont2011introduction} & 110    & 31.5      & 7044              & 4,89,938            \\ \hline
HEEAN~\cite{cheon2018bootstrapping} & 2018   & Somewhat       & Approximate           & CPU                                                     & 157    & 7,168     & 11.37                 & 1,215             \\ \hline
SEAL (BFV)~\cite{sealcrypto}              & 2019   & Somewhat       & $\times$ & $\times$                                   & 157    & 8,806   & 4,237                 & 23,954               \\ \hline
%TFHE (CPU ||)                                                & Our proposal & Fully          & Exact                 & GPU                                                     & 110    & 31.5      & 7044              & 1,74,540            \\ \hline
cuFHE~\cite{cuFHE}                                                & 2018 & Fully          & Exact                 & GPU                                                     & 110    & 31.5      & 2,032
              & 1,32,231            \\ \hline
NuFHE~\cite{NuFHE}                                                & 2018 & Fully          & Exact                 & GPU                                                     & 110    & 31.5      & 4,162
              & 1,86,011            \\ \hline
Cigulata~\cite{cingulata}                                                & 2018 & Fully          & Exact                 & $\times$                                                     & 110    & 31.5      & 2,160
              & 50,690            \\ \hline

Our Method & - & Fully          & Exact                 & GPU                                                     & 110    & 31.5      & 1,991
              & 33,930            \\ \hline
\end{tabular}
\endgroup}
% \end{adjustbox}
\color{black}
\end{table*}

==> Tables/additionComparison.tex <==
\begin{table}[]
    \centering
    
    % \caption{Execution time (in seconds) required for adding two $n$-bit numbers, where GPU$_n$ and GPU$_1$ represent the number-wise addition and bitwise addition, respectively}
    \caption{Execution time (sec) for the $n$-bit addition}% in different frameworks}%. GPU$_n$ and GPU$_1$ represent the number-wise and bitwise additions, resp.}
    \label{tbl:additionComparison}
    \begingroup
    % \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{l|c|c|c}
        \hline
        % \multirow{2}{*}{\textbf{Frameworks}} & \multicolumn{3}{c}{\textbf{Time (s)}}              \\ \cline{2-4} 
        \textbf{Frameworks}                 & \textbf{16-bit} & \textbf{24-bit} & \textbf{32-bit} \\ \hline%\hline
        Sequential                          & 3.51            & 5.23            & 7.04            \\ \hline
        cuFHE \cite{cuFHE}                              & 1.00            & 1.51            & 2.03            \\ \hline
        NuFHE \cite{NuFHE}                              & 2.92            & 3.56            & 4.16            \\ \hline
        Cingulata  \cite{cingulata}                         & 1.10            & 1.63            & 2.16            \\ \hline%\hline
        \multicolumn{4}{c}{\textbf{Our Methods}}       \\
        \hline
        CPU $\cparallel$                              & 3.51            & 5.23            & 7.04            \\ \hline
        GPU$_n\cparallel$                   & 0.94            & 2.55            & 4.44            \\ \hline
        GPU$_1\cparallel$                   & 0.98            & 1.47            & 1.99            \\ \hline
        
    \end{tabular}
    \color{black}
    \endgroup
\end{table}

==> Tables/contribSpeedup.tex <==
% \begin{table}[t]
%     \begin{center}
%         \caption{Execution time (in seconds) comparison of the our CPU and GPU  parallel framework for 32-bit numbers.[DONE]
%         \label{tab:contribution}}

%         \begin{tabular}{c|c|c|c}
%         \hline
%                 & Gate Op. & Addition & Multiplication \\ \hline
%         % BitSize & 16            & 32           & 16            & 32            & 16               & 32               \\ \hline
%         TFHE~\cite{chillotti2016faster}              & 1.40                   &   7.04                     & 489.93           \\ \hline
%         CPU-Parallel            & 0.50                   & 7.04                       & 174.54           \\ \hline
%         GPU-Parallel            & 0.10                   & 3.71                       & 59.08             \\ \hline
        
%         \end{tabular}
%     \end{center}
% \end{table}


% \begin{table}[t]
%     \centering
%     \caption{Execution time (in seconds) comparison of our CPU and GPU  parallel framework for 32-bit numbers.}
%     \label{tab:contribution}
%     \begin{tabular}{c|c|c|c}
%         \hline
%                                                               & Gate Op. & Addition & Multiplication \\ \hline
%         TFHE~\cite{chillotti2016faster} & 1.40     & 7.04     & 489.93         \\ \hline
%         CPU-Parallel                                          & 0.50     & 7.04     & 174.54         \\ \hline
%         GPU-Parallel                                          & 0.10     & 3.71     & 59.08          \\ \hline
%     \end{tabular}
% \end{table}

% \begin{table}[t]
% \caption{Execution time (in seconds, minutes for matrix multiplication) comparison of our CPU and GPU  parallel framework for 32-bit numbers (16-bit for 32$\times$32 matrix multiplication)}
% \label{tab:contribution}
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c|c}
% \hline
%                          & \multicolumn{1}{l|}{Gate Op.} & \multicolumn{1}{l|}{Add.} & \multicolumn{1}{l|}{Vector Add.} & \multicolumn{1}{l|}{Mult.} & \multicolumn{1}{l}{Mat. Mult.} \\ \hline
% % Dimension & 32-bit                            & 32-bit                        & 32-bit, 32                           & 32-bit                         & 16-bit, 32*32                           \\ \hline
% TFHE~\cite{chillotti2016faster}                     & 1.4                               & 7.04                          & 224.31                               & 489.93                         & 8717.89                                 \\ \hline
% CPU $\cparallel$             & 0.5                               & 7.04                          & 77.18                                & 174.54                         & 2514.34                                 \\ \hline
% GPU $\cparallel$             & 0.1                               & 3.71                          & 15.04                                & 59.08                          & 438.38                                  \\ \hline
% \end{tabular}
% }
% \end{table}


% \begin{table}[t]
% \caption{Execution time (in seconds, minutes for matrix multiplication) comparison of our CPU and GPU  parallel framework for 32-bit numbers (16-bit for 32$\times$32 matrix multiplication)}
% \label{tab:my-table}
% \begin{tabular}{l|c|c|c|c}
% \hline
%                                                       & \multicolumn{1}{l|}{Gate Op.} & \multicolumn{1}{l|}{Add.} & \multicolumn{1}{l|}{Mult.} & \multicolumn{1}{l}{Mat. Mult.} \\ \hline
% TFHE~\cite{chillotti2016faster} & 1.4                           & 7.04                      & 489.93                     & 8717.89                        \\ \hline
% CPU $\cparallel$                                      & 0.5                           & 7.04                      & 174.54                     & 2514.34                        \\ \hline
% GPU $\cparallel$                                      & 0.1                           & 3.71                      & 59.08                      & 438.38                         \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \caption{Execution time (in seconds) comparison of our CPU and GPU  parallel framework for 32-bit numbers. The length of the vectors for vector addition is $32$. The execution times for matrix multiplication are in minutes, and the dimension of the matrices is $32\times 32$.}
% \label{tab:my-table}
% \begin{tabular}{|l|c|c|c|c|c|}
% \hline
% &\multicolumn{1}{l|}{Gate Op.}& \multicolumn{2}{c|}{Addition} & \multicolumn{2}{c|}{Multiplication} \\ \cline{3-6} 
%                   &                                                                     & Regular        & Vector       & Regular          & Matrix           \\ \hline
% TFHE              & 1.4                                                                 & 7.04           & 224.31       & 489.93           & 8717.89          \\ \hline
% CPU $\cparallel$  & 0.5                                                                 & 7.04           & 77.18        & 174.54           & 2514.34          \\ \hline
% GPU $\cparallel$  & 0.1                                                                 & 3.71           & 15.04        & 59.08            & 438.38           \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
% \color{blue}
% \caption{A comparison of the execution times (seconds) of our CPU and GPU  parallel framework for 32-bit numbers. The length of the vectors for vector addition is $32$. The times for the matrix multiplication ($16\times 16$) are in minutes.}
\caption{A comparison of the execution times (sec) of TFHE \cite{chillotti2017faster} and our CPU, GPU  framework for 32-bit numbers }%where the addition vector lengths  are $32$
% \renewcommand{\arraystretch}{1.1}
\label{tab:contribution}
\resizebox{\linewidth}{!}{
\begingroup
% \renewcommand*{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c|c}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Gate Op.}} & \multicolumn{2}{c|}{\textbf{Addition}} & \multicolumn{2}{c}{\textbf{Multiplication}} \\ \cline{3-6} 
                  &                           & \textbf{Regular}        & \textbf{Vector}       & \textbf{Regular}          & \textbf{Matrix (mins)}           \\ \hline%\hline
TFHE~\cite{chillotti2016faster}              & 1.40                       & 7.04           & 224.31       & 489.93           & 8,717.89          \\ \hline
CPU-Parallel  & 0.50                       & 7.04           & 77.18        & 174.54           & 2,514.34          \\ \hline
GPU-Parallel  & 0.07                       & 1.99           & 11.22        & 33.93            & 186.23           \\ \hline%\hline
\end{tabular}
% \color{black}
\endgroup}
\end{table}

==> Tables/differentialTimeAnalysis.tex <==
% \begin{table*}[ht]
% \centering
% \caption{Analysis of time taken by Bootstrapping, Key switching and others for sequential and GPU-accelerated framework for different bit sizes. }
% \label{tbl:differentialtime}
% \begin{tabular}{c|l|l|l|l|l|l|l}
% \hline
% \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Sequential (CPU)}                                                                   &  & \multicolumn{3}{c}{GPU}                                                                          \\ \hline
% Bit Size               & \multicolumn{1}{c|}{Bootstrapping} & \multicolumn{1}{c|}{Key Switch} & \multicolumn{1}{c|}{Misc.} &  & \multicolumn{1}{c|}{Bootstrapping} & \multicolumn{1}{c|}{Key Switch} & \multicolumn{1}{c}{Misc.} \\ \hline
% 1                      & 0.02508205                         & 0.008043725                     & 0.000107925                &  & 0.03541062                         & 0.009758163                     & 0.000146393                \\ \hline
% 2                      & 0.05014345                         & 0.01604812                      & 8.14967E-05                &  & 0.0361374                          & 0.010127285                     & 5.474E-05                  \\ \hline
% 4                      & 0.10024168                         & 0.032073104                     & 0.000167749                &  & 0.035925733                        & 0.009946703                     & 5.93967E-05                \\ \hline
% 8                      & 0.200401371                        & 0.064059147                     & 0.000706922                &  & 0.0469246                          & 0.011191325                     & 5.5275E-05                 \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     \caption{Analysis of time (in miliseconds) taken by Bootstrapping, Key Switching and others for sequential and GPU-accelerated framework for different bit sizes ($n$).}
%     \label{tbl:differentialtime}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%         \hline
%             & \multicolumn{4}{c|}{CPU} &   & \multicolumn{4}{c}{GPU}   \\ \hline
%         $n$ &   Bootstrapping   &   Key Switch  &   Misc.   &   Total   &   &   Bootstrapping   &   Key Switch  &   Misc.   &   Total   \\ \hline
%         1   &   25.08           &   8.04        &   0.11    &   33.23   &   &   35.41           &   9.76        &   0.15    &   45.32   \\ \hline
%         2   &   50.14           &   16.05       &   0.08    &   66.27   &   &   36.14           &   10.13       &   0.05    &   46.32   \\ \hline
%         4   &   100.24          &   32.07       &   0.17    &   132.48  &   &   35.93           &   9.95        &   0.06    &   45.93   \\ \hline
%         8   &   200.4           &   64.06       &   0.71    &   265.17  &   &   46.92           &   11.19       &   0.06    &   58.17   \\ \hline
%     \end{tabular}
% \end{table*}



\begin{table*}[t]
    \centering
    % \caption{Analysis of time (millisec) for Bootstrapping, Key Switching and other operations for sequential and GPU framework \wrt different bit sizes ($n$) }
    \caption{Computation time (ms) for Bootstrapping, Key Switching and Misc. for sequential and GPU framework}
    % \renewcommand{\arraystretch}{1.1}%Though the bootstrapping time (in GPU) is similar for smaller number of bits, it gradually increases for larger bit sizes.}
    \label{tbl:differentialtime}
    \begingroup
    % \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \hline
          Bit Size  & \multicolumn{4}{c|}{\textbf{Sequential}} &   & \multicolumn{4}{c}{\textbf{GPU}}   \\ \hline
        $\textbf{n}$ &   \textbf{Bootstrapping}   &   \textbf{Key Switch}  &   \textbf{Misc.}   &   \textbf{Total}   &   &   \textbf{Bootstrapping}   &   \textbf{Key Switch}  &   \textbf{Misc.}   &   \textbf{Total}   \\ \hline%\hline
        2	&   68.89           &	17.13	    &   27.04	&   113.05	&   &   19.64   &   2.65    &   0.45    &	22.74\\ \hline
        4	&   138.02          &	34.18	    &   47.97	&   220.17	&   &   18.86   &	2.69    &	0.08    &	21.63\\ \hline
        8	&   275.67          &	68.31	    &   96.48	&   440.46	&   &   27.83   &	2.69    &	0.06    &	30.58   \\ \hline
        16	&   137.25          &	137.25	    &   425.22	&   699.72	&   &   40.70    &	2.91    &	0.44    &	44.06\\ \hline
        32	&   274.3           &	274.30	    &   852.51	&   1401.10	&   &   66.74   &	3.34    &	0.42    &	70.50\\ \hline%\hline
    \end{tabular}
    \endgroup
\end{table*}

==> Tables/linearRegressionHOST.tex <==
% 199*0.82+0.2
% 199*0.27+0.18
% 199*1.35+0.21
% 199*0.34+0.22



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\centering
% \color{blue}
\caption{Execution time (min) for Linear Regression}
\label{tbl:linearRegression}
\begin{tabular}{l|c|c|c|c}
\hline
\textbf{Datasets}                  & \textbf{\#Rows}      & \textbf{\#Attributes}  & \textbf{Data Type} & \textbf{Time} \\ \hline
\multirow{2}{*}{Dataset 1} & \multirow{4}{*}{200} & \multirow{2}{*}{10} & Numerical          & 163.38        \\ \cline{4-5} 
                           &                      &                     & Binary             & 53.91         \\ \cline{1-1} \cline{3-5}
\multirow{2}{*}{Dataset 2} &  & \multirow{2}{*}{20} & Numerical          & 268.86        \\ \cline{4-5} 
                           &                      &                     & Binary             & 67.88         \\ \hline
\multirow{2}{*}{Dataset 3} & \multirow{4}{*}{300} & \multirow{2}{*}{10} & Numerical          & 245.38        \\ \cline{4-5} 
                           &                      &                     & Binary             & 80.91         \\ \cline{1-1} \cline{3-5}
\multirow{2}{*}{Dataset 4} &  & \multirow{2}{*}{20} & Numerical          & 403.85        \\ \cline{4-5} 
                           &                      &                     & Binary             & 95.88         \\ \hline
\end{tabular}
\end{table}


==> Tables/multiplicationComparison.tex <==
\begin{table}[t]
    \centering
    % \caption{Naive and Karatsuba Multiplication runtime comparison (seconds) for $16, 24,$ and $32$-bit numbers with existing frameworks}
    \caption{Multiplication execution time (sec) comparison}% (seconds) for $16, 24,$ and $32$-bit numbers with existing frameworks}
    \label{tbl:multiplicationComparison}
    \begin{tabular}{l|c|c|c}
        \hline
        \textbf{Frameworks} & \textbf{16-bit} & \textbf{24-bit} & \textbf{32-bit} \\ \hline%\hline
        \multicolumn{4}{c}{\textbf{Naive}}                                      \\ \hline
        Sequential          & 120.64          & 273.82          & 489.94          \\ \hline
        CPU $\cparallel$     & 52.77           & 101.22          & 174.54          \\ \hline
        GPU $\cparallel$     & 11.16           & 22.08           & 33.99           \\ \hline
        cuFHE~\cite{cuFHE}               & 32.75           & 74.21           & 132.23          \\ \hline
        NuFHE~\cite{NuFHE}               & 47.72           & 105.48          & 186.00          \\ \hline
        Cingulata~\cite{cingulata}           & 11.50           & 27.04           & 50.69           \\ \hline%\hline
        \multicolumn{4}{c}{\textbf{Karatsuba}}                                  \\ \hline
        CPU $\cparallal$     & 54.76           & -               & 177.04          \\ \hline
        GPU $\cparallel$     & 7.6708          & -               & 24.62           \\ \hline%\hline
    \end{tabular}
\end{table}

==> Tables/notation.tex <==
\begin{table}[t]
    \centering
    \caption{Notations 
    %and their description 
    used throughout the paper}\label{tbl:notation}
    % \renewcommand{\arraystretch}{1.1}
    \begin{adjustbox}{max width=\columnwidth}  
    \begingroup
    % \renewcommand*{\arraystretch}{1.3}
        \begin{tabular}{c|l}
            \hline
            \textbf{Notation}            &   \textbf{Description} \\ \hline%\hline
            $\textbf{A} \in \mathbb{Z}^{r\times c}$       &   Integer matrix of dimension $r\times c$ \\ \hline
            $\overrightarrow{A} \in \mathbb{Z}^{\ell}$  &   Integer vector of length $\ell$\\ \hline
            $A, A' \in \mathbb{Z} \subset \mathbb{B}^{n}$         &   $n$-bit integer number and its complement\\ \hline
            $a_i \in \mathbb{B}$                               &   Binary bit at position $i$\\ \hline
            $\mathbb{L}^{n}$                                                &   LWE sample vector of length $n$\\ \hline
            % $A'$                                                            &   One's complement of Integer $A$\\ \hline
            $n$, $m$                                                             &   Bit size and Secret key size\\ \hline
            % $m$                                                             &   Secret key size \\ \hline
            $\cparallel$, $\ll$                                                    &   Parallel and Left Shift operation\\ \hline
            \AndGate{}{}, $|$, \XorGate{}{}                                 &   Binary AND, OR and XOR operation\\ \hline
            % $|$                                                    &   Binary OR operation\\ \hline
            % \XorGate{}{}                                                    &   Binary XOR operation\\ \hline
            % $\ll$                                                           &   Left Shift operation\\ \hline\hline
            %\hline
        \end{tabular}
        \endgroup
    \end{adjustbox}
\end{table}

==> Tables/regressionComparison.tex <==
\begin{table}[t]
\centering
\caption{Regression Analysis comparison between FV and TFHE GPU$\cparallel$ frameworks}
\label{tbl:logisticComparison}
\begingroup
\renewcommand*{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Models}}}                                        & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Ciphertext}\\ \textbf{Size (MB)}\end{tabular}}} & \multicolumn{2}{c}{\textbf{Execution Time (min)}}                                                                                                                                    \\ \cline{3-4} 
\multicolumn{1}{c|}{}                                                               & \multicolumn{1}{c|}{}                                                                           & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Numerical}\\ \textbf{Attributes}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Binary}\\ \textbf{Attributes}\end{tabular}} \\ \hline\hline
\begin{tabular}[c]{@{}l@{}}Linear Regression\\ (FV CPU $\cparallel$)\end{tabular}                     &    587.90                                                                                                 &     10.01                                                                                &           10.01                                                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Linear Regression\\ (TFHE GPU$\cparallel$)\end{tabular}   & 5.99                                                                                                &  184.95                                                                                   &     42.66                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Logistic Regression\\ (TFHE GPU$\cparallel$)\end{tabular} & 5.99                                                                                                &     189.24                                                                                &   46.77                                                                               \\ \hline\hline
\end{tabular}
\endgroup
\end{table}

==> Tables/sigmoidComparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Sigmoid Approximation comparison on different approximation models. The experimental domain includes all the data points in $[-1000, 1000]$. The error metric is Mean Square Error (MSE)}
\label{tbl:sigmoidComparison}
% \resizebox{\textwidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{1.2}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Name}                                                                              & \textbf{Deg.} & \textbf{Polynomial}                                                                                                                               & \textbf{MSE} \\ \hline\hline
\multicolumn{4}{c}{\textbf{Proposed Approximations (Piecewise)}}                                                                                                                                                                                                              \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Lagrange\end{tabular}}} & 1               & $0.125x + 0.50$                                                                                                                                     & 3.47e-05     \\ \cline{2-4} 
                                                                                           & 2               & $0.02x^2 + 0.18x + 0.432$                                                                                                                           & 1.58e-04     \\ \cline{2-4} 
                                                                                           & 3               & $0.21x - 0.006x^3 + 0.5                                                                                                                            & 1.73e-06$     \\ \hline
\textbf{Taylor}                                                                            & 3               & - $0.0005x^3 + 0.25x + 0.5                                                                                                                         & 4.05e-04$     \\ \hline
\textbf{Bernstein}                                                                         & 3               & \begin{tabular}[c]{@{}c@{}}$x^3/(exp(-1) + 1) - (x - 1)^3/2 +$ \\ $(3x(x - 1)^2)/(exp(-1/3) + 1) -$ \\ $(3x^2(t - 1))/(exp(-2/3) + 1)$\end{tabular} & 6.60e-05     \\ \hline\hline
\multicolumn{4}{c}{\textbf{Hesamifard \etal Approximation~\cite{hesamifard2018privacy}}}                                                                                                                                                                                                                   \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Chebyshev\\ Method 1\end{tabular}}}     & 3               & $-(8.60e-10)x^3 + (1.33e-17)x^2 + 0.001x + 0.499$                                                                                                       & 0.06         \\ \cline{2-4} 
                                                                                           & 5               & $(2.07e-15)x^5 - (5.32e-23)x^4 + 0.001x + 0.499$                                                                                                        & 0.72         \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Chebyshev\\ Method 2\end{tabular}}}     & 3               & $-(4.80e-10)x^3 - (7.08e-16)x^2 + 0.0009x + 0.5$                                                                                                        & 0.05         \\ \cline{2-4} 
                                                                                           & 5               & $(6.65e-16)x^5 + (9.37e-21)x^4 + 0.001*x + 0.5$                                                                                                         & 0.20         \\ \hline\hline
\end{tabular}
\endgroup
% }
\end{table*}

==> Tables/tanhComparison.tex <==
\begin{table}[]
    \centering
    \caption{Comparison of Lagrange Interpolation form for different degree}
    \label{tbl:comparisonTanh}
    \begingroup
    \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{c|c|c}
        \hline
        \textbf{Deg.} & \textbf{Polynomial}                    & \textbf{MSE} \\ \hline\hline
        1               & $0.5x$                                   & $6.97e-05$     \\ \hline
        2               & $0.16x^2 + 0.74x -0.13$ & $5.35e-04$     \\ \hline
        3               & $0.09x^3 - 0.85x$     & $0.0061$       \\ \hline\hline
    \end{tabular}
    \endgroup
\end{table}

==> algorithm/cannon.tex <==
\begin{algorithm}[t]
    \DontPrintSemicolon
    \caption{Cannon's Algorithm~\cite{cannon1969cellular}}\label{algo:cannon}
    \KwIn{\textbf{X}, \textbf{Y} $\in \mathbb{Z}^{d\times d}$}
    \KwOut{\textbf{Z} $\in \mathbb{Z}^{d\times d}$}
    \textbf{Z} = 0\;
    \For{$i \leftarrow 0$ \KwTo $d - 1$}{
        left-rotate row i of \textbf{X} by i\;
        up-rotate column i of \textbf{Y} by i\;
    %     Carry $\leftarrow$ R $\land$ B\;\label{line:addition:carryLine}
    %     R $\leftarrow$ R $\Oplus$ B\;\label{line:addition:sumLine}
    %     B $\leftarrow$ Carry $<<$ 1\;
        
    }
    \For{$k \leftarrow 0$ \KwTo $d-1$}{\label{line:cannon:seqLoopStart}
        \For{$i \leftarrow 0$ \KwTo $d-1$}{
            \For{$j \leftarrow 0$ \KwTo $d-1$}{
                $\textbf{Z}[i,j] \leftarrow \textbf{Z}[i,j] + \textbf{X}[i,j] \textbf{Y}[i,j]$\;\label{line:cannon:multiplyAdd}
            }
        }
        left-rotate of each row of $\textbf{X}$ by $1$\;
        up-rotate of each row of $\textbf{Y}$ by $1$\;
    }
    \Return{\textbf{Z}}
\end{algorithm}

==> algorithm/karatsubaMul.tex <==
\begin{minipge}
\begin{algorithm}[t]
    \DontPrintSemicolon
    \caption{Karatsuba Multiplication \cite{karatsuba1962multiplication}}\label{algo:karatsuba}
    \KwIn{X, Y $\in \mathbb{B}^n$}
    \KwOut{Z $\in \mathbb{B}^{2n}$}
    \SetKwProg{}{}{}{}
    \If{$n <n_{0}$}{
        \Return{} \FuncSty{BaseMultiplication(X, Y)}\;
    }
    % k $\leftarrow$ n/2\;
    X$_{0}\leftarrow$ X$\mod 2^{n/2}$\;
    Y$_{0}\leftarrow$ Y$\mod 2^{n/2}$\;
    X$_{1}\leftarrow$ X/2$^{n/2}$\;
    Y$_{1}\leftarrow$ Y/2$^{n/2}$\;
    
    Z$_{0} \leftarrow \FuncSty{KaratsubaMultiply}$(X$_0$, Y$_0$)\;\label{ln:karat:changeStart}
    Z$_{1} \leftarrow \FuncSty{KaratsubaMultiply}$(X$_1$, Y$_1$)\;
    Z$_{2} \leftarrow \FuncSty{KaratsubaMultiply}$(X$_0$ + Y$_0$, X$_1$ + Y$_1$)\;
    
    \Return{Z $\leftarrow$ Z$_0$ + (Z$_2$ - Z$_1$ - Z$_0$) $2^{n}$ + (Z$_1$)$2^{2n}$}\label{ln:karat:changeEnd}
\end{algorithm}
\end{minipge}

==> algorithm/minimum.tex <==
\begin{algorithm}[t]
    \DontPrintSemicolon
    \caption{Minimum of two Signed Encrypted Numbers}\label{algo:minimum}
    \KwIn{A, B $\in \mathbb{B}^{n}$}
    \KwOut{R $\in \mathbb{B}^{n+1}$}
    C = A == B \tcp*{A\:\texttt{XNOR}\:B}\label{ln:minimum:XNOR}
    $t_0$ = 0 \tcp*{$t_0$single bit}
    \For{$i \leftarrow 0$ \KwTo $n - 1$}{
        $t_0 = \: c_i \: ? \: t_0 \: : \: a_i$ \tcp*{$i^{th}$-bit of C and A}\label{ln:minimum:MUX}
    }
    % $t_0' = \: \sim t$
    $t_0 = c_{n-1}\:?\:t_0\::\:\sim t_0$\;\label{ln:minimum:lastMUX}
    R = $t_0\:?\:B\::\:A$
    
    \Return{R}
\end{algorithm}

==> algorithm/plainAddition2.tex <==
\begin{algorithm}[t]
    \DontPrintSemicolon
    \caption{Number-wise Addition}\label{algo:sequentialAddition}
    \KwIn{A, B $\in \mathbb{B}^{n}$}
    \KwOut{R $\in \mathbb{B}^{n+1}$}
    R = A\;
    \For{$i \leftarrow 0$ \KwTo $n$}{
        Carry $\leftarrow$ R $\land$ B\;\label{line:addition:carryLine}
        R $\leftarrow$ R $\Oplus$ B\;\label{line:addition:sumLine}
        B $\leftarrow$ Carry $<<$ 1
    }
    \Return{R}
\end{algorithm}

==> algorithm/plainMultiplication.tex <==
\begin{algorithm}[t]
    \DontPrintSemicolon
    \caption{Naive Multiplication}\label{algo:sequentialMultiplication}
    \KwIn{A, B $\in \mathbb{B}^{n}$}
    \KwOut{C $\in \mathbb{B}^{2n}$}
    C = 0,\:temp = 0 $\in \mathbb{B}^{2n}$\;
    \For{$i\leftarrow 0$ \KwTo $n-1$}{
        \For{$j\leftarrow 0$ \KwTo $n-1$}{\label{ln:naiveMul:andshiftStart}
        % \CommentSty{//subscripts represents bit}
        % \CommentSty{//e.g., a_i is i^{th}-bit of A}
            temp$_{j} \leftarrow$ a$_{j}\:\land\:$b$_{i}$\;
        }
        temp $\leftarrow$ temp $<<$ i\;\label{ln:naiveMul:andshiftEnd}
        C $\leftarrow$ C + temp\;
    }
    \Return{C}
\end{algorithm}

==> graphs/matrixMultiplicationTabularData.tex <==
\begin{table}[t]
    \centering
    \caption{Matrix multiplication execution time (min)}
    % \renewcommand{\arraystretch}{1.1}
    \label{tbl:matmulana}
    \begingroup
    % \renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{c|c|c|c}%|c|c|c|c}
        \hline
            % & \multicolumn{3}{c|}{16-bit}  &  & \multicolumn{3}{c}{32-bit}  \\ \hline
        \textbf{Dimension} & \textbf{Sequential} & \textbf{CPU} $\cparallel$ & \textbf{GPU} $\cparallel$ \\ \hline%\hline%&  & Sequential & CPU || & GPU || \\ \hline
        $2 \times 2$   & 17.07          & 10.62      & 0.86 \\ \hline%      &  & 0          & 0      & 0      \\ \hline
        $4 \times 4$   & 136.68         & 47.78      & 5.90 \\ \hline%      &  & 0          & 0      & 0      \\ \hline
        $8 \times 8$   & 1,090.12          & 351.82      & 43.95 \\ \hline%    &  & 0          & 0      & 0      \\ \hline
        $16 \times 16$  & 8,717.89          & 2,514.34      & 186.23  \\ \hline%\hline %    &  & 0          & 0      & 0     \\
        %$32 \times 32$  & 69733.51$^*$         & 0      & 3200.14  \\ \hline%    &  & 0          & 0      & 0     \\
    \end{tabular}
    \endgroup
\end{table}

==> graphs/vectorAdditionTabularData.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % \begin{table*}[ht]
% % \centering
% % \caption{Execution time (in seconds) taken to add vectors of different length.}
% % \label{tbl:vecAddAnaTbl}
% % \begin{tabular}{c|c|c|c|c|c|c|c}
% % \hline
% %                                                         & \multicolumn{3}{c|}{16-bit} &  & \multicolumn{3}{c}{32-bit} \\ \hline
% % \begin{tabular}[c]{@{}c@{}}Vector\\ length\end{tabular} & Sequential & OpenMP & GPU   &  & Sequential & OpenMP & GPU   \\ \hline \hline
% % 1                                                       & 2.63       & 2.66   & 1.97  &  & 5.28       & 5.29   & 4.03  \\ \hline
% % 2                                                       & 5.26       & 2.70   & 2.04  &  & 10.55      & 5.75   & 4.17  \\ \hline
% % 4                                                       & 10.54      & 3.29   & 2.38  &  & 21.11      & 6.72   & 4.89  \\ \hline
% % 8                                                       & 21.11      & 6.75   & 2.69  &  & 42.19      & 13.04  & 5.48  \\ \hline
% % 16                                                      & 42.17      & 12.86  & 3.79  &  & 84.33      & 25.84  & 7.76  \\ \hline
% % 32                                                      & 84.40      & 27.91  & 6.88  &  & 168.98     & 52.78  & 14.04 \\ \hline
% % 64                                                      & 168.63     & 57.35  & 12.53 &  & 337.63     & 107.56 & 25.47 \\ \hline\hline
% % \end{tabular}
% % \end{table*}

% \begin{table*}[]
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \hline
%                                                         & \multicolumn{3}{c|}{16-bit} &  & \multicolumn{3}{c|}{32-bit} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Vector\\ Length\end{tabular} & Sequential & OpenMP & GPU   &  & Sequential & OpenMP & GPU   \\ \hline
% 1                                                       & 2.63       & 2.66   & 1.97  &  & 5.28       & 5.29   & 4.03  \\ \hline
% 2                                                       & 5.26       & 2.70   & 2.04  &  & 10.55      & 5.75   & 4.17  \\ \hline
% 4                                                       & 10.54      & 3.29   & 2.38  &  & 21.11      & 6.72   & 4.89  \\ \hline
% 8                                                       & 21.11      & 6.75   & 2.69  &  & 42.19      & 13.04  & 5.48  \\ \hline
% 16                                                      & 42.17      & 12.86  & 3.79  &  & 84.33      & 25.84  & 7.76  \\ \hline
% 32                                                      & 84.40      & 27.91  & 6.88  &  & 168.98     & 52.78  & 14.04 \\ \hline
% 64                                                      & 168.63     & 57.35  & 12.53 &  & 337.63     & 107.56 & 25.47 \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Execution time (in seconds) taken to add vectors of different length ($\ell$).}
% \label{tbl:vecAdditionTime}
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \hline
% & \multicolumn{3}{c|}{16-bit} &  & \multicolumn{3}{c}{32-bit} \\ \hline
% $\ell$& Sequential & CPU $\parallel$ & GPU $\parallel$   &  & Sequential & CPU $\parallel$ & GPU $\parallel$   \\ \hline
% 1                                                       & 2.63       & 2.66   & 1.97  &  & 5.28       & 5.29   & 4.03  \\ \hline
% 2                                                       & 5.26       & 2.70   & 2.04  &  & 10.55      & 5.75   & 4.17  \\ \hline
% 4                                                       & 10.54      & 3.29   & 2.38  &  & 21.11      & 6.72   & 4.89  \\ \hline
% 8                                                       & 21.11      & 6.75   & 2.69  &  & 42.19      & 13.04  & 5.48  \\ \hline
% 16                                                      & 42.17      & 12.86  & 3.79  &  & 84.33      & 25.84  & 7.76  \\ \hline
% 32                                                      & 84.40      & 27.91  & 6.88  &  & 168.98     & 52.78  & 14.04 \\ \hline
% % 64                                                      & 168.63     & 57.35  & 12.53 &  & 337.63     & 107.56 & 25.47 \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
% \caption{Execution time (seconds) taken to add vectors of different length ($\ell$)}
\caption{Execution time (sec) for vector addition}
% \renewcommand{\arraystretch}{1.1}
\label{tbl:vecAdditionTime}
\resizebox{.47\textwidth}{!}{\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Length& \multicolumn{3}{c|}{\textbf{16-bit}} &  & \multicolumn{3}{c}{\textbf{32-bit}} \\ \hline
$\ell$  &   \textbf{Seq.} &   \textbf{CPU} $\cparallel$ &   \textbf{GPU} $\cparallel$ &   &    \textbf{Seq.} &   \textbf{CPU} $\cparallel$ &   \textbf{GPU} $\cparallel$ \\ \hline%\hline
%1	    &       3.52    &	    3.43        &	    1.99	    &   &       7.03    &   	6.98        &   	4.02  %  \\ \hline
%2	    &       7.06	&       3.76	    &       1.97	    &   &       14.03	&       7.65	    &       4.03    \\ \hline
4	    &       13.98	&       5.07	    &       1.27	    &   &       28.05	&       10.02	    &       2.56    \\ \hline
8	    &       27.86	&       9.96	    &       1.78	    &   &       56.01	&       19.29	    &       3.58    \\ \hline
16	    &       55.66	&       19.65	    &       2.82	    &   &       111.3	&       38.77	    &       5.70    \\ \hline
32	    &       111.32	&       38.99	    &       5.41	    &   &       224.31	&       77.18	    &       11.22    \\ \hline%\hline
\end{tabular}}
\end{table}

==> graphs/vectorMultiplicationTabularData.tex <==
% \begin{table*}[t]
% \centering
% \caption{Execution time (in minutes) taken to multiply vectors of different length ($\ell$).}
% \label{tbl:vecMultiplicationTime}
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \hline
%       & \multicolumn{3}{c|}{16-bit} &  & \multicolumn{3}{c}{32-bit} \\ \hline
% $\ell$& Sequential & CPU $\parallel$ & GPU $\parallel$   &  & Sequential & CPU $\parallel$ & GPU $\parallel$   \\ \hline
% 1      & 1.53        & 0.64   & 0.33 &  & 6.15       & 2.11   & 0.94  \\ \hline
% 2      & 3.07        & 1.75   & 0.4  &  & 12.31      & 7.35   & 1.33  \\ \hline
% 4      & 6.14        & 2.26   & 0.59 &  & 24.61      & 8.74   & 2.15  \\ \hline
% 8      & 12.28       & 4.26   & 0.97 &  & 49.22      & 17.02  & 3.77  \\ \hline
% 16     & 24.56       & 8.18   & 1.77 &  & 98.45      & 33.33  & 6.98  \\ \hline
% 32     & 49.12       & 16.08  & 3.32 &  & 196.9      & 66.76  & 13.28 \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Execution time (in minutes) taken to multiply vectors of different length ($\ell$).[IN PROGRESS]}
% \label{tbl:vecMultiplicationTime}
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \hline
%       & \multicolumn{3}{c|}{16-bit} &  & \multicolumn{3}{c}{32-bit} \\ \hline
% $\ell$& Sequential & CPU $\parallel$ & GPU $\parallel$   &  & Sequential & CPU $\parallel$ & GPU $\parallel$   \\ \hline
% 1      & 1.53        & 0.64   & 0.33 &  & 6.15       & 2.11   & 0.94  \\ \hline
% 2      & 3.07        & 1.75   & 0.4  &  & 12.31      & 7.35   & 1.33  \\ \hline
% 4      & 6.14        & 2.26   & 0.59 &  & 24.61      & 8.74   & 2.15  \\ \hline
% 8      & 12.28       & 4.26   & 0.97 &  & 49.22      & 17.02  & 3.77  \\ \hline
% 16     & 24.56       & 8.18   & 1.77 &  & 98.45      & 33.33  & 6.98  \\ \hline
% 32     & 49.12       & 16.08  & 3.32 &  & 196.9      & 66.76  & 13.28 \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[t]
\centering
% \caption{Execution time (minutes) taken to multiply vectors of different length ($\ell$)}
\caption{Execution time (min) for vector multiplication}
% \renewcommand{\arraystretch}{1.1}
\label{tbl:vecMultiplicationTime}
\resizebox{\linewidth}{!}{
\begingroup
% \renewcommand*{\arraystretch}{1.3}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
    Length   & \multicolumn{3}{c|}{\textbf{16-bit}} &  & \multicolumn{3}{c}{\textbf{32-bit}} \\ \hline
$\ell$& \textbf{Seq.} & \textbf{CPU} $\cparallel$ & \textbf{GPU} $\cparallel$   &  & \textbf{Seq.} & \textbf{CPU} $\cparallel$ & \textbf{GPU} $\cparallel$   \\ \hline%\hline
%1       &   2.02    &   0.89    &   0.32    &   &   8.15        &   2.9     &   0.97    \\ \hline
%2	    &   4.05    &   2.43	&   0.41	&   &   16.29       &   9.05    &   1.38    \\ \hline
4       &   8.13    &   3.25    &   0.41    &   &   32.56       &   12.15   &   1.61    \\ \hline
8       &   16.29   &   6.17    &   0.75    &   &   65.12       &   23.48   &   2.96    \\ \hline
16      &   32.62   &   11.93   &   1.40    &   &   130.31      &   46.39   &   5.62    \\ \hline
32      &   65.15   &   23.58   &   2.68    &   &   260.52      &   92.44   &   10.79\\ \hline%\hline
\end{tabular}
\endgroup
}
\end{table}
